Right, No Matter Why: AI Fact-checking and AI Authority in Health-related Inquiry Settings

Previous research on expert advice-taking shows that humans exhibit two contradictory behaviors: on the one hand, people tend to overvalue their own opinions undervaluing the expert opinion, and on the other, people often defer to other people's advice even if the advice itself is rather obviously wrong. In our study, we conduct an exploratory evaluation of users' AI-advice accepting behavior when evaluating the truthfulness of a health-related statement in different "advice quality" settings. We find that even feedback that is confined to just stating that "the AI thinks that the statement is false/true" results in more than half of people moving their statement veracity assessment towards the AI suggestion. The different types of advice given influence the acceptance rates, but the sheer effect of getting a suggestion is often bigger than the suggestion-type effect.

==> litrev.tex <==
\section{Related Work}
\subsection{Human decision-making in the information gathering}

\subsection{Trust in text-based decision-making systems}
\subsubsection{Calibration of trust}

\subsubsection{Quality of explanations in the AI-supporting systems}
Previous studies showed the users' need to have explanations while receiving recommendations from AI-powered systems.\cite{liao2020questioning,angerschmid2022effects}.Within the current literature, various measurement domains contribute to the issue of providing system explanations to the user \cite{mueller2021principles}. Some of these domains focus on assessing the objective outcomes of explanations, such as improving system performance or the "objective" quality of the explanation's content, including factors like understandability, fidelity, and sufficiency \cite{swartout1993explanation}, or understandability, the feeling of satisfaction, the sufficiency of detail, completeness, usefulness, accuracy, and trustworthiness \cite{muir1996trust,hoffman2023measures}. Other measures reflect the subjective metrics of user satisfaction, such as perceived trust, reliance, and also the user's understanding of the explanation.\cite{mueller2021principles}

While these objective and subjective characteristics of explanations should be interconnected, there are scenarios in which an objectively good explanation may fail to meet the user's criteria if the user's level of expertise is lower than what the system was designed for. Previous studies have shown that all modes of AI decision explanations are more or less ineffective when users have limited domain knowledge \cite{wang2021explanations}.

A more dangerous situation can appear in the reversed scenario, when the objectively bad system explanations (e.g. in the case of model hallucinations) can be assessed by the user as plausible and therefore trustworthy because of the coherent presentation, addressing the user's mental model (DO YOU HAVE ANY PART ABOUT MENTAL MODELS IN YOURS PREVIOUS CHAPTERS?)

